Finite element error analysis of wave equations with dynamic boundary conditions: $L^2$ estimates

$L^2$ norm error estimates of semi- and full discretisations, using bulk--surface finite elements and Runge--Kutta methods, of wave equations with dynamic boundary conditions are studied. The analysis resides on an abstract formulation and error estimates, via energy techniques, within this abstract setting. Four prototypical linear wave equations with dynamic boundary conditions are analysed which fit into the abstract framework. For problems with velocity terms, or with acoustic boundary conditions we prove surprising results: for such problems the spatial convergence order is shown to be less than two. These can also be observed in the presented numerical experiments.

==> packages.tex <==


\usepackage{geometry}
\geometry{a4paper,left=30mm,right=30mm, top=2.5cm, bottom=3cm}

\usepackage{mathtools}
%\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{amsmath,amssymb,amsthm}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{proposition}{Proposition}[section]

\usepackage[colorlinks=true,linkcolor=blue,urlcolor=blue,urlbordercolor={1 0 0}]{hyperref}


\usepackage{suffix} % Define commands with suffixes
\usepackage{xpunctuate}
%\usepackage{graphicx,graphics,color}
%\usepackage{epstopdf}
%\usepackage{fancyhdr}
%\usepackage{titlesec}
%\usepackage{url}

%\usepackage{mathrsfs} %nice calligraphic characters
%\usepackage{showframe}

%\usepackage{caption,subcaption}
%\usepackage{tikz}

==> texdef.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% norms and other paired delimiters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%x

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\newcommand{\ipHsymb}{m}
\DeclarePairedDelimiterX{\ipH}[2]{\ipHsymb\big\lparen}{\big\rparen}{#1, #2} % inner product in H
\DeclarePairedDelimiterXPP{\normH}[1]{}{\lvert}{\rvert}{}{#1}

\newcommand{\ipHhsymb}{m_{h}}
\DeclarePairedDelimiterX{\ipHh}[2]{\ipHhsymb\big\lparen}{\big\rparen}{#1, #2} % inner product in Hh
\DeclarePairedDelimiterXPP{\normHh}[1]{}{\lvert}{\rvert}{_{h}}{#1}
\DeclarePairedDelimiterXPP{\normHhdual}[1]{}{\lVert}{\rVert}{_{\Hh^*}}{#1}

\newcommand{\ipVsymb}{a}
\newcommand{\Vdual}{V^*}
\DeclarePairedDelimiterX{\ipV}[2]{\ipVsymb\big\lparen}{\big\rparen}{#1, #2} % inner product in V
\DeclarePairedDelimiterXPP{\normV}[1]{}{\lVert}{\rVert}{_V}{#1}
\DeclarePairedDelimiterXPP{\normVa}[1]{}{\lVert}{\rVert}{_{}}{#1}
\DeclarePairedDelimiterXPP{\normVdual}[1]{}{\lVert}{\rVert}{_{ALT,\star}}{#1}
\DeclarePairedDelimiterXPP{\normVadual}[1]{}{\lVert}{\rVert}{_{\star}}{#1}

\newcommand{\ipVhsymb}{\ipVsymb_h}
\newcommand{\Vhdual}{V_h^*}
\newcommand{\Vhl}{V_h^\ell}
\DeclarePairedDelimiterX{\ipVh}[2]{\ipVsymb_h\big\lparen}{\big\rparen}{#1, #2} % inner product in V
\DeclarePairedDelimiterXPP{\seminormVh}[1]{}{\lVert}{\rVert}{_{\sobfhsymb}}{#1}
\DeclarePairedDelimiterXPP{\normVh}[1]{}{\lVert}{\rVert}{_{h}}{#1}
\DeclarePairedDelimiterXPP{\normVhdual}[1]{}{\lVert}{\rVert}{_{\star,h}}{#1}

\newcommand{\sobfsymb}{a} % symbol for bilinear form a
\DeclarePairedDelimiterX{\sobf}[2]{\sobfsymb\big\lparen}{\big\rparen}{#1, #2} % bilinear form a
\DeclarePairedDelimiterXPP{\normVsobf}[1]{}{\lVert}{\rVert}{_{\sobfsymb}}{#1}

\newcommand{\sobfhsymb}{\sobfsymb_h} % symbol for bilinear form a_h
\DeclarePairedDelimiterX{\sobfh}[2]{\sobfhsymb\big\lparen}{\big\rparen}{#1, #2} %  discrete bilinear form a_h
\newcommand{\sobfBsymb}{b} % symbol for bilinear form a
\DeclarePairedDelimiterX{\sobfB}[2]{\sobfBsymb\big\lparen}{\big\rparen}{#1, #2} % bilinear form a
\newcommand{\sobfBhsymb}{\sobfBsymb_h} % symbol for bilinear form a
\DeclarePairedDelimiterX{\sobfBh}[2]{\sobfBhsymb\big\lparen}{\big\rparen}{#1, #2} % bilinear form a
\newcommand{\DeltaipHsymb}{\Delta\ipHsymb} % error form inner product
\DeclarePairedDelimiterX{\DeltaipH}[2]{\DeltaipHsymb\big\lparen}{\big\rparen}{#1, #2} % bilinear form 
\newcommand{\DeltaipVsymb}{\Delta\ipVsymb} % error form inner product
\DeclarePairedDelimiterX{\DeltaipV}[2]{\DeltaipVsymb\big\lparen}{\big\rparen}{#1, #2} % bilinear form 
\newcommand{\Deltasobfsymb}{\Delta\sobfsymb} % error form differential operator
\DeclarePairedDelimiterX{\Deltasobf}[2]{\Deltasobfsymb\big\lparen}{\big\rparen}{#1, #2}
\newcommand{\DeltasobfBsymb}{\Delta\sobfBsymb} % error form differential operator
\DeclarePairedDelimiterX{\DeltasobfB}[2]{\DeltasobfBsymb\big\lparen}{\big\rparen}{#1,
  #2}  % bilinear form 


\DeclarePairedDelimiterX{\dpV}[2]{\langle}{\rangle_V}{#1,#2}

\DeclarePairedDelimiterXPP{\norminf}[2]{}{\lVert}{\rVert}{_{L^\infty\left( #2 \right)}}{#1}
\DeclarePairedDelimiterXPP{\normsup}[2]{}{\lVert}{\rVert}{_{\infty,#2}}{#1}
\DeclarePairedDelimiterXPP{\col}[1]{}{\lparen}{\rparen}{}{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathematical operators 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lift}[1]{#1^\ell}
\newcommand{\intpo}{\widetilde I_h}
\newcommand{\intpol}{I_h}
\newcommand{\Ritz}{\widetilde R_h}
\newcommand{\Ritzl}{R_h}
\newcommand{\RitzlB}{R_h^\Om}
\newcommand{\RitzlS}{R_h^\Ga}
\newcommand{\dotr}{\mbox{$\boldsymbol{\cdot}$}}
\newcommand{\defeq}{=}
\newcommand{\leqC}{\lesssim}
\newcommand{\ot}{\leftarrow}
\newcommand{\dembd}{\overset{d}{\hookrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathematical operators 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\FEbulk}{S_h}
\newcommand{\FEsurf}{S_h^\Gamma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% variables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%texdef for bcs 
\input{bcsTexDef}


\newcommand{\soiv}{u_0} % second order initial value
\newcommand{\sois}{u_1} % second order initial speed
\newcommand{\sosrc}{f} % second order source term
\newcommand{\so}{\sor} % 2nd order linear operator
\newcommand{\soinv}{\sor^{-1}} % 2nd order linear operator
\newcommand{\sor}{A} % 2nd order linear operator restricted to H
\newcommand{\soB}{\soBr} % 2nd order linear operator
\newcommand{\soBr}{B} % 2nd order linear operator restricted to H


\newcommand{\soivh}{\intpo \soiv} % second order initial value
\newcommand{\soish}{\intpo \sois} % second order initial speed
\newcommand{\sods}{V_h} % second order discrete space
\newcommand{\sosrch}{\intpo \sosrc}
\newcommand{\sorh}{\sor_h} % discrete 2nd order operator 
\newcommand{\sorhinv}{\sor_h^{-1}} % discrete 2nd order operator 
\newcommand{\soBrh}{\soBr_h} % discrete 2nd order operator 

\newcommand{\defect}{d_h}

\newcommand{\solift}{Q_h^V}
\newcommand{\liftH}{\solift}
\newcommand{\liftV}{\solift}

\newcommand{\los}{\mathcal{L}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% constants
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cGard}{c_G} % \constant from Garding inequality
\newcommand{\cGardh}{\widehat c_{G}} % \constant from Garding inequality
\newcommand{\cqmb}{\rho_{\textnormal{qm}}}
\newcommand{\cqmbh}{\widehat{\rho}_{\textnormal{qm}}}
\newcommand{\ccoerc}{\alpha}
\newcommand{\ccoerch}{\^\alpha}
\newcommand{\CH}{C_H} % norm equivalence constant
\newcommand{\cH}{c_H} % norm equivalence constant
\newcommand{\CV}{C_V} % norm equivalence constant
\newcommand{\cV}{c_V} % norm equivalence constant
\newcommand{\cHhVh}{C_{\ipHhsymb,\ipVhsymb}} % V-H-embedding constant (inverse inequality)
\newcommand{\cHhsobfh}{C_{\ipHhsymb,\sobfhsymb}} % V-H-embedding constant (inverse inequality)
\newcommand{\cexp}{\lambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathematical terms and abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\BC}{boundary conditions}
\newcommand{\dynBC}{dynamic boundary condition}
\newcommand{\SD}{semi-discretisation}
\newcommand{\SOWEQ}{second-order wave equation}
\newcommand{\WEQ}{wave equation}
\newcommand{\CSI}{Cauchy--Schwarz inequality}
\newcommand{\FE}{finite element}
\newcommand{\FEM}{finite element method}
\newcommand{\PDE}{partial differential equation}

% abbreviations
\newcommand{\eg}{e.g\xperiod}
\newcommand{\ie}{i.e\xperiod}
\newcommand{\cf}{cf\xperiod}
\newcommand{\wrt}{w.r.t\xperiod}
%\newcommand{\st}{s.t\xperiod}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbV}{\mathbb V}
\newcommand{\Hh}{H_h}
\newcommand{\uh}{u_h}
\newcommand{\vh}{v_h}
\newcommand{\wh}{w_h}
\newcommand{\ui}{u_1}
\newcommand{\uii}{u_2}
\newcommand{\vi}{v_1}
\newcommand{\vii}{v_2}
\newcommand{\wi}{w_1}
\newcommand{\wii}{w_2}
\newcommand{\uhi}{u_{h,1}}
\newcommand{\uhii}{u_{h,2}}
\newcommand{\vhi}{v_{h,1}}
\newcommand{\vhii}{v_{h,2}}
\newcommand{\whi}{w_{h,1}}
\newcommand{\whii}{w_{h,2}}
\newcommand{\Landau}{\mathcal O}
\newcommand{\eps}{\varepsilon}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 		some usual macros of Christian and Balázs
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\bfa{{\mathbf a}}
\newcommand\bfb{{\mathbf b}}
\newcommand\bfc{{\mathbf c}}
\newcommand\bfd{{\mathbf d}}
\newcommand\bfe{{\mathbf e}}
\newcommand\bff{{\mathbf f}}
\newcommand\bfk{{\mathbf k}}
\newcommand\bfp{{\mathbf p}}
\newcommand\bfq{{\mathbf q}}
\newcommand\bfr{{\mathbf r}}
\newcommand\bfu{{\mathbf u}}
\newcommand\bfw{{\mathbf w}}
\newcommand\bfx{{\mathbf x}}
\newcommand\bfy{{\mathbf y}}
\newcommand\bfz{{\mathbf z}}
\newcommand\bfA{{\mathbf A}}
\newcommand\bfC{{\mathbf C}}
\newcommand\bfD{{\mathbf D}}
\newcommand\bfE{{\mathbf E}}
\newcommand\bfF{{\mathbf F}}
\newcommand\bfG{{\mathbf G}}
\newcommand\bfH{{\mathbf H}}
\newcommand\bfI{{\mathbf I}}
\newcommand\bfL{{\mathbf L}}
\newcommand\bfM{{\mathbf M}}
\newcommand\bfS{{\mathbf S}}
\newcommand\bfT{{\mathbf T}}
\newcommand\bfX{{\mathbf X}}
\newcommand\bfZ{{\mathbf Z}}
\newcommand\bfalpha{{\boldsymbol \alpha}}
\newcommand\bfbeta{{\boldsymbol \MU}}
\newcommand\bfmu{{\boldsymbol \mu}}
\newcommand\bfomega{{\boldsymbol \omega}}
\newcommand\bfOmega{{\boldsymbol \Omega}}
%\newcommand\bfPsi{{\boldsymbol \Psi}}
\newcommand\bfzero{{\mathbf 0}}
\newcommand\calJ{{\cal J}}
\newcommand\calK{{\cal K}}
\newcommand\calU{{\cal U}}
\newcommand\calH{{\cal H}}
\newcommand\calF{{\cal F}}
\newcommand\calN{{\mathcal N}}
\newcommand\calR{{\mathcal R}}
\newcommand\calP{{\mathcal P}}
\newcommand\calQ{{\mathcal Q}}
%+1
\newcommand\for{\quad\hbox{ for}\quad }
\newcommand\with{\quad\hbox{ with}\quad }
%
\renewcommand\Re{\mathrm{Re}\,}
\renewcommand\ss{s}
%\renewcommand\d{\textrm{z}}
%\newcommand\dt{\tau}
\newcommand\tp{{\tt T}}

\newcommand\calE{{\cal E}}
\newcommand\calT{{\mathcal T}}
\newcommand{\bfvphi}{\boldsymbol{\varphi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bflambda}{\boldsymbol{\lambda}}
\newcommand{\bfDelta}{\boldsymbol{\Delta}}
\newcommand{\dimOm}{d}
\def \S     {\mathcal{S}}
\newcommand{\bfv}{\boldsymbol{v}}


%% macros
\newcommand{\A}{\mathcal{A}}
\newcommand{\andquad}{\qquad \textrm{ and } \qquad}
\newcommand{\co}{continuous}
\DeclareMathOperator{\dop}{d}
\def \d {\mathrm{d}}
\newcommand{\disp}{\displaystyle}
\renewcommand{\div}{\textnormal{div}\hspace{2pt}}
\newcommand{\Ga}{\Gamma}
\newcommand{\gr}{gradient}
\newcommand{\Id}{\textrm{Id}}
\newcommand{\inv}{^{-1}}
\newcommand{\la}{\langle}
\newcommand{\laplace}{\Delta}
\newcommand{\lin}{linear}
\newcommand{\lm}{{\rm LM}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\nb}{\nabla}
\newcommand{\Om}{\Omega}
\newcommand{\Omh}{\Omega_h}
\newcommand{\op}{operator}
\newcommand{\pa}{\partial}
\newcommand{\R}{\mathbb{R}}
\newcommand{\ra}{\rangle}
\newcommand{\re}{\textnormal{Re}}
\newcommand{\resp}{respectively}
\newcommand{\spn}{\textnormal{span}}
\newcommand{\st}{such that}
\def \t {(t) }
\def \to {\rightarrow}
\newcommand{\vphi}{\varphi}
%\def \nu {\textnormal{n}}

%+1
\newcommand\quadand{\quad\hbox{ and }\quad}
\newcommand\quadwith{\quad\hbox{ with }\quad}
\newcommand\quadfor{\quad\hbox{ for }\quad}
\newcommand\quadfore{\quad\hbox{ for every }\quad}
%
\newcommand{\ccdot}{(\cdot,\cdot)}
\newcommand{\ee}{\textnormal{e}}
\newcommand{\diff}{\tfrac{\d}{\d t}}
\newcommand{\half}{{\tfrac{1}{2}}}
\newcommand{\Half}{{\frac{1}{2}}}

%% surface related definitons
\newcommand{\ga}{\gamma}
\newcommand{\nbg}{\nb_{\Ga}}
\newcommand{\nbgh}{\nb_{\Ga_h}}

%% review/reviewing related defintions
\def\bbk{\color{blue}}
\def\ebk{\color{black}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros from Karlsruhe 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Big comment environment
\newcommand{\TODO}[1]{%
    \smallskip {\color{red} \hrule \vspace*{1mm}
    \textbf{\underline{To-Do:}} #1 \vspace*{1mm}
    \hrule} \vspace*{1mm}
}

%Small comment environment.
\WithSuffix\newcommand\TODO*[1]{{\color{red}#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% margin todo macro
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\todo}[2]{\textcolor[rgb]{1.00,0.00,0.00}{{#2}}\vspace{-0.4201109cm}\marginpar{{\footnotesize [todo: #1]}}\vspace{1.0042cm}}


